Uniqueness of discrete solutions of nonmonotone PDEs without a globally fine mesh condition

Uniqueness of the finite element solution for nonmonotone quasilinear problems of elliptic type is established in one and two dimensions. In each case, we prove a comparison theorem based on locally bounding the variation of the discrete so- lution over each element. The uniqueness follows from this result, and does not require a globally small meshsize.

==> makefile <==
#! make
##############################################################################
# Purpose: MCP (Mathematical and Computational Physics Group) paper makefile.
#
# Notes:   This makefile is used by the MCP group (Michael Holst's Research 
#          Group in the Mathematics and Physics Departments at UC San Diego)
#          to build latex papers using the fairly simple combination of 
#          pdflatex, amstex/amslatex, and pdf/png images.
#
# Targets: The makefile will auto-generate the following based on the
#          requested make target:
#
#            Main Targets:
#
#              pdfth   --> ${TARGET}.pdf via pdflatex
#              pdf     --> ${TARGET}.pdf via pdflatex + thumbpdf
#              dvi     --> ${TARGET}.dvi via latex
#              dvip    --> ${TARGET}.dvi|ps|pdf via latex + dvips + ps2pdf
#
#            Auxilliary Targets:
#
#              arx     --> zarxiv.tar.gz (gzipped tarball for arXiv)
#              clean   --> rm -f *.aux, *.dvi, etc
#              rclean  --> clean + rm *.ps *.bbl (careful!)
#              rrclean --> rclean + rm m.pdf mm.pdf ${TARGET}.pdf (careful!)
#
# Author:  Michael Holst
# Date:    Sat Dec 19 22:23:18 PST 2009
##############################################################################

default: pdf

TARGET=PoZh17a

ARXIV_DIR=zarxiv
ARXIV_FILES=${TARGET}.tex ${TARGET}.bbl \

LATEX=latex
PDFLATEX=pdflatex
#PDFLATEX=pdflatex --shell-escape
BIBTEX=bibtex
#BIBTEX=./zbibtex

all : pdf arx

dvi :
	make clean
	${LATEX} ${TARGET}.tex
	-${BIBTEX} ${TARGET}
	${LATEX} ${TARGET}.tex
	${LATEX} ${TARGET}.tex
	-cp -f ${TARGET}.dvi mm.dvi

dvip : dvi
	dvips -N0 -P pdf -t letter -o ${TARGET}.ps mm.dvi
	ps2pdf ${TARGET}.ps
	-cp -f ${TARGET}.pdf mm.pdf

pdf :
	make clean
	${PDFLATEX} ${TARGET}
	-${BIBTEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	-cp -f ${TARGET}.pdf mm.pdf

pdfth : pdf
	thumbpdf ${TARGET}
	${PDFLATEX} ${TARGET}
	rm -f thumb*.png
	-cp -f ${TARGET}.pdf mm.pdf

arx : ${TARGET}.bbl
	./makex ${ARXIV_DIR} ${ARXIV_FILES}

clean :
	rm -f *.aux *.dvi *.log *.lof *.lot *.toc *.blg *.idx *.out *.tpt

rclean :
	make clean
	rm -f *.ps *.bbl

rrclean :
	make rclean
	rm -f m.pdf mm.pdf ${TARGET}.pdf
	rm -rf ${ARXIV_DIR}


